Foundational Models in Medical Imaging: A Comprehensive Survey and Future Vision

Foundation models, large-scale, pre-trained deep-learning models adapted to a wide range of downstream tasks have gained significant interest lately in various deep-learning problems undergoing a paradigm shift with the rise of these models. Trained on large-scale dataset to bridge the gap between different modalities, foundation models facilitate contextual reasoning, generalization, and prompt capabilities at test time. The predictions of these models can be adjusted for new tasks by augmenting the model input with task-specific hints called prompts without requiring extensive labeled data and retraining. Capitalizing on the advances in computer vision, medical imaging has also marked a growing interest in these models. To assist researchers in navigating this direction, this survey intends to provide a comprehensive overview of foundation models in the domain of medical imaging. Specifically, we initiate our exploration by providing an exposition of the fundamental concepts forming the basis of foundation models. Subsequently, we offer a methodical taxonomy of foundation models within the medical domain, proposing a classification system primarily structured around training strategies, while also incorporating additional facets such as application domains, imaging modalities, specific organs of interest, and the algorithms integral to these models. Furthermore, we emphasize the practical use case of some selected approaches and then discuss the opportunities, applications, and future directions of these large-scale pre-trained models, for analyzing medical images. In the same vein, we address the prevailing challenges and research pathways associated with foundational models in medical imaging. These encompass the areas of interpretability, data management, computational requirements, and the nuanced issue of contextual comprehension.

==> sections/discussion.tex <==
\section{Discussion}
In the dynamic landscape of foundational models for medical imaging, each direction outlined in our taxonomy (\Cref{fig:taxonomy}) brings its own set of advantages and distinctive capabilities to the forefront. These divergent paths cater to specific needs, creating a diversified toolkit for addressing the multifaceted challenges of the medical imaging domain. As we delve into this discussion, we'll explore the unique advantages of each direction and consider scenarios where one direction might excel over the others, all while peering into how these models learn feature representations and the implications thereof.

\noindent \textbf{Textually Prompted Contrastive Models}:
These models have shown remarkable prowess in bridging the semantic gap between medical images and text. By leveraging contrastive learning, these models can extract meaningful representations from unpaired medical image-text data, thereby reducing the dependence on vast amounts of labeled data. This approach is particularly advantageous in scenarios where labeled data is scarce or expensive to obtain, such as rare medical conditions or specialized imaging modalities. Contrastive models excel at capturing subtle medical meanings and are well-suited for tasks like zero-shot prediction in medical image-text tasks. For instance, in scenarios where a new, uncharacterized medical condition arises, these models can adapt swiftly by simply providing textual descriptions.

However, there are limitations to consider. Contrastive models might struggle with highly complex medical images or intricate pathologies, where the nuances demand a deeper level of feature representation. Additionally, they may still rely on the availability of large-scale text data, which could be a bottleneck in some cases. The contrastive learning process also hinges on careful tuning of hyperparameters, making it essential to invest time in fine-tuning for optimal performance.

\noindent \textbf{Textually Prompted Generative Models}:
Textually prompted generative models, exemplified by models like Clinical-BERT \citep{yan2022clinical} and Med-Flamingo \citep{moor2023med}, offer the ability to generate detailed responses and explanations for medical image-related queries. They excel in tasks requiring a deep understanding of the medical domain, making them invaluable in clinical decision support systems, medical education, and generating radiology reports.

These generative models can be a game-changer when interpretability and reasoning are crucial. For instance, in a clinical setting, generating explanations for a model's predictions can enhance trust and facilitate collaboration between AI systems and medical professionals. In educational contexts, they can serve as powerful tutors, providing in-depth explanations and context.

Nevertheless, generative models are computationally intensive and demand significant training data. They may not be the most efficient choice for scenarios where quick, lightweight predictions are required. Additionally, they may face challenges in generating text that is both informative and concise, which could be important in some applications.

\noindent \textbf{Textually Prompted Hybrid Models}:
Hybrid models, as represented by MedBLIP \citep{chen2023medblip}, combine the strengths of generative and contrastive methodologies. These models tackle the challenge of integrating textual data with 3D medical images, often a complex task due to the inherent differences in data modalities.

One of the key advantages of hybrid models is their potential for zero-shot prediction in medical image-text tasks. They seamlessly align visual attributes with linguistic features, making them adept at executing medical visual question-answering tasks with precision. For example, in cases where medical professionals need to quickly diagnose conditions based on both images and textual descriptions, hybrid models can provide valuable support.

Yet, hybrid models may face challenges related to the design of effective integration mechanisms between textual and visual data. The success of these models often relies on the quality of the alignment between different modalities. Additionally, they may require substantial computational resources for training and fine-tuning.

            
\noindent \textbf{Textually Prompted Conversational Models}:
Conversational models, like LLaVA-Med \citep{li2023llava} and XrayGPT \citep{thawkar2023xraygpt}, are designed to enable interactive dialogues between medical professionals and AI systems. These models are particularly beneficial in scenarios where medical experts need to ask questions, seek explanations, or instruct AI systems regarding medical images.
One of the most significant advantages of conversational models is their potential to enhance communication and collaboration between humans and AI. They can facilitate knowledge transfer, clarify doubts, and provide detailed explanations for complex medical images. In a clinical context, this can lead to more informed decision-making and better patient care.

However, conversational models face the challenge of understanding context and handling ambiguous queries effectively. Ensuring accurate responses in complex medical scenarios remains an ongoing research challenge. Additionally, they require careful fine-tuning on conversational datasets to perform optimally.


\noindent \textbf{Visually Prompted Adaptations Models}:
Visually prompted adaptations models, such as MedLSAM \citep{lei2023medlsam}, MedLSAM, 3DSAM-adapter \citep{gong20233dsam}, SAM-Med2D \citep{cheng2023sammed2d}, SAMed \citep{zhang2023customized}, and SAM-U \citep{deng2023samu}, focus on enhancing the specificity and performance of medical image segmentation tasks. These models adapt foundational models like SAM for the medical domain, addressing challenges like data scarcity and complex boundaries. A sample of segmentation results on various medical image analysis tasks achieved through the adapted SAM model is presented in \Cref{fig:discussion-prove}, showcasing its remarkable achievement in diverse medical imaging scenarios and its robust generalization power.

% >>>>>>>>>>>>>>>>>> TABLE >>>>>>>>>>>>>>>>>>>>
\include{overview-table}
% <<<<<<<<<<<<<<<<<< TABLE <<<<<<<<<<<<<<<<<<<<

The primary advantage of adaptation models is their ability to excel in specialized medical image segmentation tasks. For instance, in scenarios where precise tumor volume calculation is critical, models like MedSAM can provide accurate results. These models are tailored for the medical domain, making them well-suited for specific clinical applications.

Nonetheless, adaptation models may require substantial annotated data for fine-tuning. They might face challenges in scenarios with limited labeled data, as achieving the desired level of performance could be challenging. Additionally, they might not be the most efficient choice for tasks that require generalization across diverse medical imaging modalities.

\noindent \textbf{Visually Prompted Generalist Models}:
Visually prompted generalist models, exemplified by models like BiomedGPT \citep{zhang2023biomedgpt} and Med-PalM M \citep{tu2023generalist}, offer versatility by handling a wide spectrum of medical imaging tasks and data modalities. They can seamlessly switch between tasks without the need for extensive retraining, making them suitable for dynamic healthcare environments.

The key advantage of generalist models is their flexibility. In scenarios where medical professionals need a single model that can handle various tasks, such as image classification, text generation, and question-answering, these models shine. Their ability to reason across different modalities and provide informed responses is invaluable in clinical decision support and medical research.

However, generalist models might face challenges related to task-specific fine-tuning. Achieving state-of-the-art performance in highly specialized tasks might require additional domain-specific data. Moreover, these models need robust mechanisms for handling out-of-distribution data effectively.

In conclusion, the choice between these directions largely depends on the specific use case and requirements. While textually prompted models excel in tasks requiring interpretation and detailed explanations, visually prompted models dominate in segmentation and image-specific tasks. Conversational models bridge the gap between human experts and AI systems, facilitating collaborative decision-making. The choice ultimately boils down to the nature of the problem, the availability of data, and the need for adaptability or versatility in the medical imaging domain. Each direction contributes to the evolving landscape of foundational models, offering a rich tapestry of tools to tackle diverse healthcare challenges. 
To facilitate comprehension, we have presented the benefits, drawbacks, and practical applications of each direction in \Cref{tab:paperhighlights}. 
We also showcase the timeline of the reviewed papers in the past quarters, as illustrated in \Cref{fig:timeline}.
This figure presents a chronological overview of the key milestones and developments in the field, highlighting the rapid evolution and growing significance of textually prompted and visually prompted foundation models in medical imaging. Expanding on this, the timeline provides valuable insights into the progression of research, revealing the emergence of novel techniques, conversational, and generalist models. 


\begin{figure*}[!thb]
\centering
\includegraphics[width=0.7\textwidth]{Figures/timeline.pdf}
\caption{Timeline of advancements in textually and visually prompted foundation models in medical imaging over the past quarters." This timeline illustrates significant progress and breakthroughs in the field, spanning the last five quarters, highlighting the dynamic nature of research and innovation in textually and visually prompted foundation models for medical image analysis.}
\label{fig:timline}
\end{figure*}








==> sections/introduction.tex <==

\section{Introduction}
\label{intro}
Foundation Models (FMs) refer to artificial intelligence (AI) models that exhibit notable progress in their development. These models are typically trained on extensive, diverse datasets, often utilizing self-supervision techniques at a massive scale. Following this initial training, they can be further adapted, such as through fine-tuning, for a wide array of downstream tasks that are related to the original training data \citep{bommasani2021opportunities}.

In contrast to the conventional deep learning paradigm, which heavily relies on large-scale, task-specific, and crowd-labeled data for training individual deep neural networks (DNNs) for various visual recognition tasks, FMs offer a more efficient alternative. They are pre-trained on large-scale datasets that are nearly limitless in availability, allowing for direct application to downstream tasks with only a limited amount of labeled data. This shift in approach holds the promise of significantly reducing the labor and time traditionally required for such tasks.
The recent surge can be traced back to the growth facilitated by the rise of large language models (LLMs) and the expansion of data and size \citep{awais2023foundational}. Models such as GPT-3 \citep{brown2020language}, PaLM \citep{chowdhery2022palm}, Galactica \citep{taylor2022galactica}, and LLaMA \citep{touvron2023llama} have exhibited strong capacities to understand natural language and solve complex tasks with zero/few-shot learning, attaining remarkable results without the need for extensive task-specific data.
Concurrently, large vision foundation models make rapid progress in perception tasks \citep{jia2021scaling,yao2021filip} where a vision-language model (VLM) is pre-trained with large-scale image-text pairs and the Pre-trained VLM can be directly applied to downstream visual recognition tasks. VLMs generally consist of three fundamental parts: textual feature, visual feature, and fusion module. These elements work together in harmony, allowing the models to proficiently utilize text and visual data to produce logical and contextually appropriate results. Specifically, the pre-training of VLMs typically follows certain vision-language objectives, which facilitate the acquisition of image-text correlations from extensive collections of image-text pairs. For instance, the pioneer study CLIP \citep{schuhmann2021laion}, an image-text matching
model utilizes contrastive learning methods to create combined representations for images and texts where the learning goal is to minimize the gap between the representation of an image-text pair, while simultaneously increasing the separation between representations of unrelated pairs. Besides this so-called ``\emph{\textbf{Textually Prompted Models (TPMs)}}", a line of research has investigated FMs with where visual inputs (points, boxes, masks) can prompt which we refer to ``\emph{\textbf{Visually Prompted Models (VPMs)}}" \citep{awais2023foundational} (See \cref{fig:models} for a visual depiction of both.). The seminal Segment Anything (SA) model \citep{kirillov2023segment} sparked huge attention in the vision community recently. SAM stands as a promptable model crafted for the purpose of broad image segmentation, trained over 1 billion masks on 11 million images using a promptable segmentation task that enables powerful zero-shot generalization. Furthermore, the SAM model undergoes expansion and further refinement through training on a substantial dataset encompassing 4.6 million medical images along with 19.7 million corresponding masks \citep{cheng2023sammed2d}. This dataset offers a rich diversity, spanning 10 distinct medical data modalities, and includes annotations for 4 anatomical structures in addition to lesions. Impressively, it comprehensively represents 31 major human organs. This augmented training regimen has yielded noteworthy results, particularly in terms of bolstering the model's capacity for enhanced generalization.


Moreover, this generic visual prompt-based segmentation model has recently adapted to a wide range of downstream tasks, e.g., medical image analysis \citep{ma2023segment,lei2023medlsam}, image inpainting \citep{yu2023inpaint}, style transfer \citep{liu2023any}, and image captioning \citep{wang2023caption} to name a few. Apart from foundational models that rely on textual and visual prompts, research endeavors have also delved into creating models aimed at harmonizing various paired modalities (such as image-text, and video-audio) to learn representations assisting diverse downstream tasks.

The inception of foundation models has attracted tremendous attention to rethink the development of medical AI systems \citep{ji2023continual,zhang2023text,wang2023foundation,nguyen2023lvm}. Despite significant progress in biomedical AI, task-specific models continue to be the primary methodologies employed, however, medicine is essentially multimodal, with rich data modalities spanning text, imaging, genomics, and more \citep{tu2023generalist}. Inherently, a \emph{Medical Foundation Model (MFM)} has the ability to adaptively interpret a variety of medical modalities, encompassing diverse data sources such as images, electronic medical records, lab findings, genomic information, medical diagrams, and textual data \citep{moor2023foundation}.
Hence, foundational models could potentially offer an enhanced foundation for tackling immediate clinical issues, advancing the field of medical imaging, and enhancing the effectiveness and efficiency of disease diagnosis and treatment enabling the possibility of building a unified biomedical AI system that can interpret multimodal data with complex structures. With the acceleration of both biomedical data production and advancements, the influence of these models is set to expand by an influx of contributions (As \Cref{fig:evolution} illustrates that there exists a significant body of research dedicated to the application of FMs in diverse medical imaging contexts till the first release of our survey, October 2023.), encompassing a wide array of potential applications that range from fundamental biomedical discovery to the improvement of healthcare delivery. Hence, conducting a review of the current literature would be beneficial for
the community and quite timely. 

\begin{figure*}[!thb]
\centering
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/charts/chart-algs}
         \caption{Algorithms}
         % \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/charts/chart-mods}
         \caption{Modalities}
         % \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/charts/chart-organs}
         \caption{Organs}
         % \label{fig:y equals x}
     \end{subfigure}
\caption{The diagram (a) displays the distribution of published papers categorized by their applications, while (b) categorizes them by their imaging modalities. Additionally, (c) denotes the count of research papers in the medical domain that are based on foundational models. The year-over-year growth rate underscores the increasing significance of diffusion models in future research. It's worth noting that the total number of papers included in the analysis is 100.}
\label{fig:graphs}
\end{figure*}

This paper provides a holistic overview of the foundation models developed for medical imaging applications. We distinguish existing works inspired by the taxonomy proposed in \citep{awais2023foundational} and highlight the major strengths and shortcomings of the existing methods. We hope this work will
point out new paths, provide a road map for researchers, inspire further interest, and ignite additional enthusiasm within the vision community leveraging the potential of foundation models in the medical discipline. This survey will be regularly updated to reflect the dynamic progress of the MFMs, as
this is a rapidly evolving and promising field towards AGI in the biomedical field. Our major contributions include:

$\bullet$~We conduct a thorough and exhaustive examination of foundation models proposed in the field of medical imaging, beginning from background and preliminaries for foundation models, to specific applications along with the
organ concerned and imaging modality in a hierarchical and structured manner

$\bullet$~Our work provides a taxonomized (\cref{fig:charts}), in-depth analysis (e.g. task/organ-specific research progress and limitations), as well as a discussion of various aspects.

$\bullet$~Furthermore, we discuss the challenges and unresolved aspects linked to foundation models in medical imaging. We pinpoint new trends, raise important questions, and propose future directions for further exploration.



\begin{figure}[!ht]
	\centering
	\includegraphics[width=.8\columnwidth]{Figures/fig-models.pdf}
    \caption{Visual illustration of how our extensive classification categorizes existing works into textually and visually prompted models, distinct from traditional vision models.}
    \label{fig:models}
\end{figure}
 


\begin{figure*}[!thb]
\centering
\includegraphics[width=\textwidth]{Figures/taxonomy.pdf}
\caption{\textcolor{red}{
    The suggested taxonomy for foundational models used in medical imaging research consists of six distinct groups: I) VPM-Generalist, II) TPM-Hybrid, III) TPM-Contrastive, IV) TPM-Generative, V) VPM-Adaptations, and VI) TPM-Conversational. To maintain conciseness, we assign ascending prefix numbers to each category in the paper's name and cite each study accordingly as follows:} \input{taxonomy-references.tex}
}
\label{fig:taxonomy}
\end{figure*}


\textbf{Clinical Importance.}
In medical imaging, foundation models are reshaping the way research methods are designed and paradigms are approached, paving the way for innovative advancements and pioneering breakthroughs across various sectors owing to some of their inherent properties aligned with the medical domain as follows. 
\textbf{Multi-Modality.} Despite advances in biomedical AI, most models today are limited to single-task, unimodal functions. For instance, a mammogram interpretation AI excels at breast cancer screening but can't incorporate patient records, and additional data like MRI, or engage in meaningful dialogue, limiting its real-world applicability. 
\textbf{Explainability and Generalization.} The absence of explainability in deep learning models can erode trust among clinicians accustomed to clear clinical insights. The ability of models to generalize across different medical settings is vital due to varying data sources. Foundation models address these issues by offering a unified framework for tasks like detection and classification, often trained on diverse datasets from various medical centers, enhancing their potential for clinical use by ensuring interpretability and broad applicability. 
\textbf{Privacy Preservation.} The computer vision community has a history of open-sourcing datasets, but in medical imaging, privacy regulations limit data sharing. Foundation models offer a privacy-preserving alternative by allowing knowledge transfer without direct access to sensitive data. Additionally, federated learning enables model training on distributed data while keeping it on local machines, ensuring data privacy. Moreover, foundation models facilitate privacy preservation by generating synthetic data resembling real medical images, eliminating the need for actual patient data in model training.
\textbf{Addaptability} Existing medical AI models struggle when faced with distribution shifts caused by changes in technology, procedures, settings, or populations. In contrast, MFMs can effectively adapt to these shifts through in-context learning. For instance, a hospital can teach an MFM model to interpret X-rays from a new scanner by providing a few examples as prompts, enabling it to adjust to new data distributions in real time. This capability is mainly seen in large language models and is not common in conventional medical AI models, which would typically require complete retraining with new datasets.
\textbf{Domain Knowledge} Unlike clinicians, traditional medical AI models often lack initial medical domain knowledge, relying solely on statistical associations. Medical imaging foundation models like GMAI can address this limitation by integrating formal medical knowledge, using structures like knowledge graphs and retrieving relevant context from existing databases, improving their performance on specific tasks.
In summary, foundation models play a crucial role in advancing medical applications by providing a robust and adaptable framework that enhances efficiency, generalizability, and privacy preservation. Their ability to support various clinical tasks and promote collaboration makes them invaluable tools for improving patient care and medical research.

\textbf{Relevant Surveys.}
With the recent success of foundation models, there has
been a surge of surveys and contributions in this domain.
Some of the reviews investigate recent advances
in LLMs, distinguishing different aspects of LLMs by analyzing the impact of pre-training adaptation tuning, utilization, and evaluation \citep{zhao2023survey,fan2023bibliometric,huang2022towards}. In the context of vision models, the work of \citep{awais2023foundational} provides a comprehensive review of FMs including their typical architecture design, training objectives, and prompting mechanisms. The work of \citep{gu2023systematic} delivers a comprehensive survey of research in prompt engineering on diverse types of vision-language models, organizing existing prompt-engineering approaches from a new perspective. Besides, \citep{zhang2023vision} provides a systematic review of visual language models for various visual recognition tasks including image classification, object detection, and semantic segmentation.
In the medical imaging field, \citep{moor2023foundation} identifies the potential applications, opportunities, and challenges of MFMs. The work of \citep{shi2023generalist} provides a comprehensive and objective evaluation of SAM on medical image segmentation, while \citep{zhang2023challenges} discusses the spectrum, and future directions of foundation models.
However, different from the aforementioned works, we devise a multi-perspective taxonomy of foundation models in the medical community, providing a systematical category of research in medical foundation models and their applications dividing them into textually prompted models, and visually prompted models where each paper is broadly classified according to the proposed algorithm along with the organ concerned and imaging modality, respectively. We present the concepts and theoretical foundations behind foundation models ranging from training objectives and instruction-aligning to prompt engineering (\Cref{sec:background}). In \Cref{sec:textual} to \Cref{sec:other}, we comprehensively cover an extensive and up-to-date overview of the recent medical foundation models, as shown in \Cref{fig:tasks}. We wrap up this survey by pinpointing future directions and open challenges facing foundation models in medical imaging in \Cref{sec:challenge}.

\textbf{Search Strategy.}
We conducted extensive searches across various platforms, such as DBLP, Google Scholar, and Arxiv Sanity Preserver. We leveraged their search capabilities to create tailored queries and compile comprehensive lists of academic works. These searches encompassed a broad spectrum of scholarly publications, including peer-reviewed journal articles, conference papers, workshop materials, non-peer-reviewed content, and preprints. We tailored our search criteria to achieve this diversity. Our specific search queries consisted of keywords \texttt{(foundation* $|$ generalist* $|$ medical* $|$ \textbf{\{Task\}}*), (med-\textbf{\{FM\}} $|$ foundation*), (foundation* $|$ biomedical* $|$ image* $|$ model*)}, where \textbf{\{FM\}} and \textbf{\{Task\}} refer to one well-known vision foundation model(such as \textit{PaLM}, \textit{CLIP}, etc) or Tasks (such as \textit{Segmentation}, \textit{Question Answering}, etc) in medical imaging. We then applied filtering to eliminate false positives, ensuring that only papers related to foundation models were included in our analysis.

\textbf{Paper Organization.}
The rest of the survey is organized as follows. \Cref{sec:background} presents the background and preliminaries for foundation models. We adopt the taxonomy of \citep{awais2023foundational} and categorize previous studies into two main groups: those prompted by textual inputs (discussed in \cref{sec:textual}) and those driven by visual cues (discussed in \cref{sec:visual}). In the context of textually prompted foundation models, we further subdivide them into contrastive, generative, hybrid (combining contrastive and generative approaches), and conversational visual language models. In addition, we differentiate textually prompted models into adaptations and generalist models. Furthermore, \Cref{sec:challenge} reveals the risk, open problems, and
future directions of foundation models. Finally, we conclude our research in \Cref{sec:conclusion}.



==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:background}

The term "foundational models" made its debut at Stanford Institute for Human-Centred AI in \citep{bommasani2021opportunities} with the definition of \emph{"the
base models trained on large-scale data in a self-supervised or
semi-supervised manner that can be adapted for several other
downstream tasks"}. Specifically, inspired by the surge of large language models (LLMs), using the basic fundamentals of deep learning such as DNNs and self-supervised learning, foundation models have emerged by massively scaling up both data and model size. 
In this section, we introduce the basic model architectures, concepts, and settings behind FMs focusing on contributing factors for these models in computer vision such as training
objectives, instruction-aligning, inference procedure and prompting.

\subsection{Pre-training Objectives}
\label{sec:objective}
Diverse pretraining objectives have been devised to learn a rich understanding of the relationship between vision and language \citep{mu2021slip,9878693,he2020momentum,radford2021learning}. We broadly categorize them into contrastive and generative objectives.

\subsubsection{Contrastive Objectives}

Contrastive objectives instruct models to acquire distinctive representations \citep{chen2020simple,he2020momentum} by bringing related sample pairs closer together while pushing unrelated pairs farther apart within the feature space. Specifically, \textbf{\textit{Image Contrastive Loss (ICL)}} aims to learn discriminative image features making a query image closely resemble its positive keys (i.e., its data augmentations) while ensuring it remains distant from its negative keys (i.e., other images) within the embedding space. Consider a batch of $B$ images, contrastive objectives such as InfoNCE \citep{Oord2018RepresentationLW} and its variations \citep{he2020momentum,chen2020simple}, $\mathcal{L}_{\text{I}}^{\text{InfoNCE}}$ can be expressed as:

\[
\mathcal{L}_{\text{I}}^{\text{InfoNCE}} = -\frac{1}{B} \sum_{i=1}^B \log \frac{\exp\left(\theta_i^{\text{query}} \cdot \theta_{+}^{\text{positive}} / \tau\right)}{\sum_{j=1, j \neq i}^{B+1} \exp\left(\theta_i^{\text{query}} \cdot \theta_j^{\text{key}} / \tau\right)}
\]

where, $\theta_i^{\text{query}}$ represents the query embedding, $\{\theta_j^{\text{key}}\}_{j=1, j \neq i}^{B+1}$ are the key embeddings, where $\theta_{+}^{\text{positive}}$ denotes the positive key corresponding to $\theta_i^{\text{query}}$, while the rest are considered negative keys. The hyperparameter $\tau$ governs the density of the learned representation.

\textbf{\textit{Image-Text Contrastive Loss (ITCL)}}
Seeks to develop distinctive image-text representations by bringing together the embeddings of matched images and texts and pushing apart those that do not match \citep{radford2021learning,jia2021scaling}.
Let $\left(i, t_i\right)$ represent the $i$-th image-text example, then, the image-to-text loss is calculated as:

\[
\mathcal{L}_{I \rightarrow T} = -\log \left[\frac{\exp \left(\theta_i \cdot \theta_{+} / \tau\right)}{\sum_{j=1}^N \exp \left(\theta_i \cdot \theta_j / \tau\right)}\right]
\]

where $N$ is the total number of such pairs, and $\theta_i$ corresponds to the embedding for image $i$, while $\theta_{+}$ and $\theta_j$ denote positive and negative text representations, respectively. The losses are computed with a focus on the relationship between images and texts while considering the temperature parameter $\tau$.

The text-to-image loss is also calculated similarly, and the total loss is the sum of these two terms:

    

\[
\mathcal{L}_{ITC} = \frac{1}{N} \sum_{i=1}^N \left[\mathcal{L}_{I \rightarrow T} + \mathcal{L}_{T \rightarrow I}\right]
\]

Akin to \textit{ICL} and \textit{ITCL}, various contrastive loss functions have also found an application (\textbf{SimCLR} \citep{chen2020simple,DBLP:conf/nips/ChenKSNH20}, \textbf{FILIP Loss} \citep{Yao2021FILIPFI}, \textbf{Region-Word Alignment (RWA)} \citep{li2022grounded}, and \textbf{Region-Word Contrastive (RWC)} \citep{zhang2022glipv2}).

\subsubsection{Generative Objectives}
Generative objectives involve teaching networks to produce image or text data, which allows them to acquire semantic features, accomplished through tasks like image generation \citep{Bao2021BEiTBP}, and language generation \citep{Liu2019RoBERTaAR}.

\textbf{\textit{Masked Image Modelling (MIM)}} 
involves the acquisition of cross-patch correlations by applying masking and image reconstruction techniques. In MIM, a selection of patches within an input image is randomly masked, and the encoder is trained to reconstruct these masked patches based on the unmasked patches. For a given batch of $B$ images, the loss function is formulated as:

\[
\mathcal{L}_{MIM} = -\frac{1}{B} \sum_{i=1}^B \log f_\theta\left(\bar{x}_i^I \,|\, \hat{x}_i^I\right),
\]

where $\bar{x}_i^I$ and $\hat{x}_i^I$ represent the masked and unmasked patches within $x_i^I$, respectively \citep{zhang2023vision}.


\textbf{\textit{Masked Language Modelling (MLM)}} is a widely adopted pretraining objective in Natural Language Processing (NLP). In MLM, a specific percentage of input text tokens is randomly masked, and these masked tokens are reconstructed using the unmasked ones. The loss function for MLM can be expressed as:

\[
\mathcal{L}_{MLM} = -\frac{1}{B} \sum_{i=1}^B \log f_\theta\left(\bar{x}_i^T \,|\, \hat{x}_i^T\right),
\]

where $\bar{x}_i^T$ and $\hat{x}_i^T$ denote the masked and unmasked tokens within $x_i^T$, respectively, and $B$ denotes the batch size \citep{zhang2023vision}.

Likewise, diverse additional generative loss functions have been introduced in the field including Masked Multimodal Modeling (MMM) loss \citep{singh2022flava}, Image-conditioned Masked Language Modeling (IMLM) loss \citep{zhang2023toward}, and Captioning with Parallel Prediction (CapPa) \citep{tschannen2023image}.

\subsection{Pre-training Tasks}

As discussed in \cref{sec:objective}, FMs pre-training has been studied with typical approaches including contrastive objectives, and generative objectives. In natural language processing, certain pre-training tasks include masked language modeling, where words in the input sequence are randomly hidden, and the model predicts these hidden words during pre-training. Another task involves next-sentence-prediction, where pairs of sentences from distinct documents are presented, and the model determines whether the order of these sentences is accurate. Additionally, there's the denoising auto-encoder task, which introduces noise into the original text corpus and then aims to reconstruct the pristine input using the noisy version of the corpus.
Likewise, to enable the generalization of learned representations to a range of downstream vision domains, pretext tasks such as inpainting \citep{wang2023images}, auxiliary supervised discriminative tasks, and data reconstruction tasks \citep{luo2023segclip} are used in the pre-training stage.

\subsection{Instruction-Aligning}

Instruction-aligning methods aim to let the LM follow human intents and generate meaningful outputs. This process involves either fine-tuning the model on a diverse set of tasks with human-annotated prompts and feedback (RLHF) \citep{ouyang2022training}, conducting supervised fine-tuning on publicly available benchmarks and datasets, which are augmented with manually or automatically generated instructions, and improving the reasoning ability
of LLMs by instructing them to produce a sequence of intermediate actions that ultimately lead to the solution of a multi-step problem (Chain-of-thought) \citep{bai2022constitutional}.

\subsection{Prompt Engineering}

Prompt engineering refers to a method that enhances a large pre-trained model by incorporating task-specific hints, referred to as prompts, to tailor the model for new tasks 
enabling the power to acquire
predictions based only on prompts without updating model parameters \citep{gu2023systematic}.
In the context of large language models (LLMs) prompting techniques can be categorized into two primary groups depending on the clarity of the templates they employ: "soft prompts" (optimizable, learnable) and "hard prompts (manually crafted text prompts)". Within the "hard prompt" category, there are four subcategories: task instructions, in-context learning, retrieval-based prompting, and chain-of-thought prompting. In contrast, "soft prompts" fall into two strategies: prompt tuning and prefix token tuning, which differ in whether they introduce new tokens into the model's architecture or simply attach them to the input. 
In the vision domain, prompt engineering facilitates the acquisition of joint multi-modal representations (e.g., CLIP \citep{radford2021learning} for image classification of ALIGN \citep{Li2021AlignBF}) to introduce human interaction to the foundational models and employs vision-language models for visual tasks.






